Mitigating Biases for Instruction-following Language Models via Bias Neurons Elimination

Instruction-following language models often show undesirable biases. These undesirable biases may be accelerated in the real-world usage of language models, where a wide range of instructions is used through zero-shot example prompting. To solve this problem, we first define the bias neuron, which significantly affects biased outputs, and prove its existence empirically. Furthermore, we propose a novel and practical bias mitigation method, CRISPR, to eliminate bias neurons of language models in instruction-following settings. CRISPR automatically determines biased outputs and categorizes neurons that affect the biased outputs as bias neurons using an explainability method. Experimental results demonstrate the effectiveness of our method in mitigating biases under zero-shot instruction-following settings without losing the model's task performance and existing knowledge. The experimental results reveal the generalizability of our method as it shows robustness under various instructions and datasets. Surprisingly, our method can mitigate the bias in language models by eliminating only a few neurons (at least three).

==> texts/intro_prev.tex <==
\input{fig_texts/fig1}

Instruction-following language models perform various tasks using instruction-based prompts \citep{chung2022scaling, touvron2023llama, taori2023alpaca, openai2023gpt4}.
However, language models have suffered from undesirable biases, failing to follow user instructions despite their significant competency \citep{tamkin2021understanding, weidinger2021ethical, bender2021dangers, bommasani2021opportunities}.
Figure~\ref{fig:intro1} shows an example of undesirable biases in an instruction-following language model for a minor group.
In this case, an instruction-following language model assigns a high probability to a minor group for a negative question despite the ambiguity of the given context.

Furthermore, instruction-following language models tend to show perceptual biases when understanding instructions.
Figure~\ref{fig:intro2} shows the inconsistent behavior of the Flan-T5-base in various synonymous instructions on BBQ-SES \citep{parrish2021bbq} and MRPC \citep{wang2018glue} datasets.
This result indicates that a language model is easily distracted by varying instructions despite given semantically the same instructions.
These two phenomena suggest that language models exhibit significant cognitive biases in instruction settings.

Existing studies \citep{zhao2021calibrate, fei2023mitigating} have investigated and mitigated several label biases under few-shot in-context learning settings.
Specifically, they have regarded the imbalanced probability distribution that occurred by inputting content-free texts (e.g., "N/A" or random tokens) as biases, and degraded the original output probability of each input instance by the output probability of the content-free texts.
% However, the previous studies have not fundamentally eliminated biases since they have simply shifted the output probability of each data equally, only considering the label biases.
% To fundamentally eliminate bias in processing each data, bias elimination at the neuron level is necessary.
However, they have only aimed to mitigate biases in few-shot in-context learning settings, not considering the zero-shot instruction prompting.
Since utilizing a language model in only the instruction prompting without few-shot examples is an efficient and practical usage scenario of language models, they have significant limitations in the scope of application.



\input{fig_texts/fig2}


In this paper, we define the \textbf{\textit{bias neuron}}, which significantly influences inferring biased outputs in language models and prove its existence empirically.
Furthermore, we propose a novel bias mitigation method called \textbf{CRISPR}, which stands for \textbf{C}alib\textbf{R}ating \textbf{I}n\textbf{S}truction Bias via Bias Neuron \textbf{PR}uning.
We utilize an attribution \citep{yang2023task}, an explainability method for language models, to quantify the bias of each neuron at three levels: (1) token level, (2) text level, and (3) instruction level.
Specifically, we first compute the token level bias influence in inferring a predefined biased output, and aggregate the token level score to a text and instruction level hierarchically to derive the final bias influence (\textit{bias attribution}) of each neuron.
Furthermore, defining biased outputs manually for each data sample is time-consuming; thus, we propose an automatic identification method of biased outputs for computing the bias attribution using the confusion score of a language model.

% Experimental results show that our method effectively mitigates biases under the zero-shot instruction prompting settings.
% We demonstrate our method for social bias and natural language understanding benchmarks and dramatically increase the performance of instruction-following language models.

We demonstrate our method for social bias and natural language understanding benchmarks and dramatically mitigates the biases of language models in zero-shot instruction settings.
In contrast, baseline methods fail to mitigate biases in zero-shot instruction settings.
Surprisingly, we observe that only a few bias neurons (e.g., three neurons) cause the bias, and we prove that significantly few neurons affect the undesirable behavior of language models.
Furthermore, we reveal that mitigating bias for a particular task does not adversely affect the existing knowledge of other tasks within the language models.
In addition, we note that the bias knowledge is transferred to datasets from correlative domains by showing that bias neurons identified for a specific dataset also function as biases in other analogous datasets.
CRISPR is a notably practical debiasing method since it needs only a few data samples (i.g., ten samples) to quantify the bias score for the whole neurons.
CRISPR also enables language models to adapt flexibly by eliminating some existing bias neurons without any training process.
